VizGenie: Toward Self-Refining, Domain-Aware Workflows for Next-Generation Scientific Visualization

We present VizGenie, a self-improving, agentic framework that advances scientific visualization through large language model (LLM) by orchestrating of a collection of domain-specific and dynamically generated modules. Users initially access core functionalities--such as threshold-based filtering, slice extraction, and statistical analysis--through pre-existing tools. For tasks beyond this baseline, VizGenie autonomously employs LLMs to generate new visualization scripts (e.g., VTK Python code), expanding its capabilities on-demand. Each generated script undergoes automated backend validation and is seamlessly integrated upon successful testing, continuously enhancing the system's adaptability and robustness. A distinctive feature of VizGenie is its intuitive natural language interface, allowing users to issue high-level feature-based queries (e.g., ``visualize the skull"). The system leverages image-based analysis and visual question answering (VQA) via fine-tuned vision models to interpret these queries precisely, bridging domain expertise and technical implementation. Additionally, users can interactively query generated visualizations through VQA, facilitating deeper exploration. Reliability and reproducibility are further strengthened by Retrieval-Augmented Generation (RAG), providing context-driven responses while maintaining comprehensive provenance records. Evaluations on complex volumetric datasets demonstrate significant reductions in cognitive overhead for iterative visualization tasks. By integrating curated domain-specific tools with LLM-driven flexibility, VizGenie not only accelerates insight generation but also establishes a sustainable, continuously evolving visualization practice. The resulting platform dynamically learns from user interactions, consistently enhancing support for feature-centric exploration and reproducible research in scientific visualization.

==> README <==
Created by Torsten Moeller, April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016
modified by Cagatay Turkay and Soumya Dutta, September 2019
modified by Cody Dunne, January and March 2023

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used with an established LaTeX environment by calling pdfLaTeX or LaTex. For online collaborative editing or without a local LaTeX installation, one option is to use https://www.overleaf.com/. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Unix-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> obsolete/methodology1.tex <==
\subsection{Automated Agentic Workflows via User Specifications}

Motivated by the recent developments in agentic workflows powered by more capable LLMs (that can produce high quality code), and also recent trend in LLM-based workflows for generating scientific visualization generation (such as ChatVis\cite{mallick:2025:chatvis}), we initially proposed to explore a purely automated agentic workflow leveraging large language models (LLMs) to dynamically generate and execute code in response to every user requested natural language instructions. Our developed such automated agentic system operated in a constrained local environment with access limited to a single directory and basic shell commands (e.g., ls, curl, pip, and Python execution). Agents interact with the LLM via the OpenAI API, sending descriptions and local file contexts to generate code, execute it locally, and iteratively refine based on results and errors. All software tools and visualizations are built dynamically at runtime, without reliance on preinstalled packages. A dedicated security agent evaluates generated code and commands for potential risks before execution, ensuring safe and controlled operation. This setup enables flexible, just-in-time software synthesis for exploration and analysis within a secure and self-contained environment.

While this approach showed promise in its flexibility and autonomy, it also presents several limitations. Relying on dynamically generated software for all tasks, particularly in domains like data visualization, can be inefficient compared to using mature, industry-standard tools that offer stability, performance, and refined user experiences. Additionally, we observed that the system achieved \textit{successful} outcomes in only about $50\%$ of our trials: identical prompts often led to varied implementations with different trade-offs in quality, accuracy, and utility. These inconsistencies prompted us to explore a more prescriptive and task-specific approach, which we detail in the next section.

\subsection{Vizman Agent47: Visualization-aware Agentic Workflow}

Vizman Agent47 is designed as a hybrid system that combines a static set of robust visualization tools with the flexibility of dynamic module generation via large language models (LLMs). By leveraging natural language interfaces, the system interprets user queries and orchestrates a pipeline that transforms high-level instructions into concrete visualization outputs. Our workflow is characterized by iterative refinement and continuous self-improvement, ensuring that the system adapts to evolving user needs and domain-specific challenges.

\subsubsection{Agent Setup via Tool Access}
To support the diverse requirements of Vizman Agent47, we designed a multi-model architecture that employs several specialized large language models (LLMs), each tuned for a specific class of tasks. At the core of our system, a primary LLM is used to orchestrate overall workflow decisions. The LLM isconfigured with a deterministic setting (temperature = 0) and for this initial work, the \texttt{gpt-4o} model has been chosen. This choice ensures that high-level planning and agent coordination remain consistent and reliable, a critical factor when managing complex, multi-step visualization pipelines.

For general-purpose interactions that demand unambiguous and context-aware responses, we also employ an instance of the same \texttt{gpt-4o} model. This consistency across general tasks minimizes variability and helps maintain a coherent conversational context. 
In contrast, the initial code generation tasks are handled by an LLM configured with a higher temperature (set to 1) and based on the \texttt{o3-mini} model. This configuration encourages creative and diverse outputs, which is beneficial when synthesizing new visualization scripts that might need to incorporate novel solutions or adapt to previously unseen user queries. 
However, when it comes to modifying code, where precision is paramount, we utilize a smaller, more focused model (\texttt{gpt-4o-mini}) with a deterministic setting. This variant is specifically tuned to generate concise and accurate code modifications without the risk of unnecessary creativity that might introduce errors. This setting balances the interaction time vs quality. (A detailed study on these choices can be found in the Results and Discussion Section.)

The overall orchestration of these models is managed by a zero-shot agent framework based on the \texttt{zero-shot-react-description} paradigm. This approach was selected over other agent architectures because it facilitates flexible, on-the-fly reasoning without requiring extensive prior training for every new task. Alternatives, such as few-shot or fine-tuned agents, might offer improvements in specialized contexts but often at the cost of reduced generality and increased development overhead. In our design, the zero-shot setup, combined with a robust callback manager and an integrated conversation buffer for maintaining context, allows Vizman Agent47 to seamlessly transition between diverse tasks while preserving a complete provenance of interactions.

Together, this multi-LLM setup and the chosen agent framework ensure that Vizman Agent47 can robustly handle everything from high-level task orchestration to fine-grained code modifications. The deliberate selection of model configurations for each subtask strikes a balance between determinism and creativity, enabling the system to generate reliable visualizations while adapting dynamically to complex, domain-specific queries.


\subsubsection{Data Set Related Queries with Added Context}

Vizman Agent47 supports sophisticated data set queries by leveraging context-aware tools that integrate local metadata with domain expertise. In particular, the \texttt{SimulationInfo} tool is designed to provide general information about the available data, answering questions such as “How many different data sets do I have?” or “What are the characteristics of these simulation runs?” This tool reads a file containing the folder structure and details of the simulation data (e.g., in VTK/ParaView-readable format), and then constructs a prompt that encapsulates this local context. 

The constructed prompt explicitly instructs the LLM to act as an expert in scientific visualization for high-performance simulation codes, particularly in VTK and ParaView workflows. By including the raw text from the local data list, the system ensures that the LLM is not operating solely on generic knowledge but is also informed by the specifics of the available data. This contextual grounding significantly improves the relevance and accuracy of the responses. For instance, when a user asks about the number of datasets or specific attributes of a simulation run, the LLM can reference the detailed folder structure to provide an answer that is both precise and tailored to the user's environment.

Users can optionally add more context to the data sets by adding a README file to the folder and adding the path of the file in the optional comment column of the file. This extra context information can further improve the LLMs ability to answer data-related questions.

This design not only mitigates ambiguity in the queries but also enriches the interaction by embedding domain-specific details into the response generation process. As a result, users receive detailed, contextually informed answers that help guide further exploration and analysis within the Vizman Agent47 framework.


\subsubsection{Pre-existing Tools vs Dynamically Generated Modules}

Vizman Agent47 is designed with a dual approach that combines a set of robust, pre-existing tools with the flexibility to generate new modules on demand. The pre-existing tools—such as \texttt{FilterRuns}, \texttt{VisualizeRun}, and \texttt{AnalyzeRuns}—are implemented to perform routine operations. For example, \texttt{FilterRuns} applies threshold-based filtering on simulation data, \texttt{VisualizeRun} extracts and displays 2D slices from volumetric datasets, and \texttt{AnalyzeRuns} computes key statistical metrics across simulation runs. These tools are thoroughly validated and serve as a stable baseline for common queries, ensuring that everyday visualization tasks are handled reliably and efficiently.

In contrast, when user queries demand capabilities beyond the baseline—for instance, specialized 3D rendering, novel feature extraction, or any visualization task that is not covered by the pre-existing toolkit—Vizman Agent47 leverages the \texttt{CodeGenerator} module. This module accepts inputs in the form of a JSON object containing a textual prompt (which specifies the desired modifications or enhancements) along with a reference to the data set. The system then uses an LLM-based coder to dynamically generate VTK Python code that adheres to a prescribed structure, 
% including a function named \texttt{update\_vtk\_scene(renderer)} 
for integrating the new visualization routines. To ensure reliability and traceability, the generated code is logged into a SQLite database along with its associated prompt and identified visualization type. This database also assists in improving system's response time in the future by acting as a system cache [See Code Validation below].
This process not only expands the system’s functionality but also provides a mechanism for incremental improvement and long-term evolution.

The deliberate design choice to integrate both pre-existing tools and dynamically generated modules enables Vizman Agent47 to maintain a robust, reproducible baseline while simultaneously adapting to the evolving, domain-specific requirements of its users. This hybrid strategy is fundamental to our contribution, as it combines stability with extensibility—ensuring that the system can reliably perform standard tasks while also learning and incorporating new visualization capabilities as needed.


\subsubsection{Full Code Regeneration vs Incremental Code Updates}

A central challenge in automated scientific visualization is striking the right balance between full code regeneration and incremental code updates. Vizman Agent47 addresses this challenge through a dual mechanism: for tasks that require a completely new visualization approach, the system triggers full code regeneration via the \texttt{CodeGenerator} tool. This module generates new VTK Python code based on detailed natural language prompts and contextual information from the data, ensuring that novel visualization requirements can be met from scratch. Full code regeneration is particularly useful when the visualization task is substantially different from previous requests or when existing modules do not support the desired functionality.

In contrast, many visualization tasks involve modifying or fine-tuning an already generated module—for instance, changing a colormap, adjusting an isovalue, or refining a visualization parameter. To address these scenarios, we developed the \texttt{ModifyGeneratedCode} tool. This tool accepts a JSON input containing the modification instructions along with optional file parameters. It first loads the current code from the specified file, constructs a prompt that instructs the LLM to only make necessary modifications without rewriting the entire module, and then invokes the LLM to generate the updated code. A key design constraint is that any changes to the function declaration must remain backward compatible—ensuring that previous code invocations remain valid. 

The integration of both full code regeneration and incremental updates offers a flexible solution. The system leverages full regeneration when facing entirely new tasks, while relying on incremental updates to refine existing modules efficiently. This dual approach minimizes redundancy, preserves validated functionality, and reduces the risk of introducing new errors. As a result, Vizman Agent47 not only adapts dynamically to diverse visualization challenges but also ensures robustness and continuity over time.

\subsubsection{Code Validation}

A critical component of Vizman Agent47 is ensuring that every generated visualization module meets the required functionality and executes without errors. To achieve this, our system integrates a dedicated code validation tool that operates in two stages: validation and, optionally, iterative fixing.

When a new module or VTK code is generated by the LLM, it is stored in a persistent database (by default, \texttt{code\_generation\_log.db}). This database not only archives the generated code but also logs its status using a state indicator (0 for not validated, 1 for validated with no errors, 2 for validated with errors not fixed, and 3 for validated with errors fixed). Initially, the status flag remains 0 if the code was interactively generated by the user. As we use a "reasoning model" for code generation (e.g., "o3-mini"), generally the quality of the code at the initial stage is still quite high. We chose to perform the validation on the unvalidated code at user's request or at the backend, to keep the system response time interactive (as much as possible).

When the code validation tool is invoked, this tool first retrieves the most recent prompt and the corresponding generated code from the code database.
The retrieved code is then written to a designated output file and executed. The system captures both standard output and any runtime errors during execution. Subsequently, a validation prompt is constructed by combining the original user requirements (as specified in the prompt), the generated code, and the runtime outputs and errors. This comprehensive prompt is sent to an LLM with coding capabilities (e.g., we just reuse "o3-mini" in our workflow for this purpose) which evaluates whether the code meets 1. user specified requirements as described in the prompt, 2. operates correctly and has no execution issues. If the response indicates missing features or errors, the feedback is used to decide whether the code needs further modifications.

When any issues are found with the code (either missing features or execution errors), the system enters an iterative fixing phase. During this phase, the LLM is prompted with the current code along with the validation feedback, and it generates an updated version that attempts to address the identified issues. The modified code is then re-executed and re-evaluated. This loop repeats for a predefined number of iterations (e.g., up to three), with the goal of converging on a version of the code that satisfies all user requirements and runs without error. Finally, the tool updates the corresponding entry in the database with the final validation state, providing a robust audit trail and ensuring reproducibility.

This rigorous code validation and self-correction mechanism is central to our approach. It not only guarantees that the dynamically generated modules are functional and reliable but also enhances the system's ability to adapt to complex, domain-specific visualization tasks by continuously refining its output.

\subsubsection{Feature-based Query for Scientific Data}

One of the most critical and innovative capabilities of Vizman Agent47 is its support for high-level, feature-based queries that require deep domain insight. Rather than limiting users to generic data queries, our system empowers them to ask complex, feature-specific questions such as “Show me the skull for dataset X” or “Visualize the boundaries of the region of interest.” To accomplish this, Vizman Agent47 combines advanced image space analysis, a structured knowledge base, and LLM-based reasoning—all enhanced by a locally fine-tuned Llama-Vision model.

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{tvcg-journal-latex-2024.02.09/figs/word-distribution-skull.png}
        \caption{skull}
        \label{fig:word-distributions-skull}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{tvcg-journal-latex-2024.02.09/figs/word-distribution-nasal.png}
        \caption{nasal}
        \label{fig:word-distributions-nasal}
    \end{subfigure}
    ~ 
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{tvcg-journal-latex-2024.02.09/figs/word-distribution-teeth.png}
        \caption{teeth}
        \label{fig:word-distributions-teeth}
    \end{subfigure}
    \caption{The mean term frequency of each anatomical term increases and distributions widen after processing with the VQA pipeline, resulting in better isovalue determination and image retrieval. Means are represented by white triangles, medians by white circles.}
    \label{fig:word-distributions}
\end{figure*}

\textbf{Image Space Analysis via Specialized Vision Models: Brad/Shawn}
The process begins with the automated generation of screenshots for each dataset. Multiple views are captured from different camera angles, and key metadata (e.g., computed isovalues and textual descriptions) are extracted from each image using our vision question-answering (VQA) pipeline. This VQA component leverages a locally fine-tuned Llama-Vision model, which has been optimized for scientific imagery, to analyze each screenshot and generate precise, domain-relevant descriptions. The resulting metadata—comprising isovalue measurements and feature descriptions—is then stored in a dedicated SQLite database, creating a rich, searchable repository of visualization contexts. After applying the VQA pipeline, we see in Figure \ref{fig:word-distributions} that it improves the distributions of key terms \emph{skull}, \emph{nasal}, and \emph{teeth} corresponding to the examples shown in Figure \ref{fig:sys_view_teaser}. These differences are also statistically significant at p < 0.05 when applying the nonparametric Mann-Whitney U test, demonstrating the additional value of the VQA pipeline to improving results.

\begin{tcolorbox}[colback=gray!10, colframe=black, title=Prompt to the Vision Model for Each Screenshot, sharp corners]
"Given the context: \{context\}"\\[1ex]
"What features do you see in this image? Provide a succinct answer assuming that this image shows an isosurface from a scientific data set."
\end{tcolorbox}


\textbf{Interactive Feature-based Query Support:}
When a user issues a feature-based query, Vizman Agent47 first queries the SQLite database to retrieve candidate entries corresponding to the requested feature. These entries include both the isovalues used during the generation of the screenshots and the accompanying natural language descriptions derived from the vision model. The system then constructs a summary prompt that aggregates these candidate details and employs an LLM to determine the most appropriate isovalue that is likely to extract the desired feature from the dataset. This step is critical because it ensures that the selected isovalue is informed not only by raw numerical data but also by the nuanced, visually derived descriptions provided by the Llama-Vision model.

\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{tvcg-journal-latex-2024.02.09/figs/interface_Screenshot_annotated.png}
    \caption{ A screenshot of our designed chat interface for our agentic workflow.}
    \label{fig:chat_view}
    % \vspace{-1em}
\end{figure*}

\textbf{Feature Visualization:}
Once the optimal isovalue is identified, Vizman Agent47 uses it to either modify an existing visualization module or generate a new VTK Python code snippet tailored to highlight the feature. This adaptive process can involve incremental code updates—adjusting parameters such as isovalue thresholds and colormap settings—or complete code regeneration when the feature extraction requirements differ significantly from prior modules. The integration of these steps guarantees that even subtle and complex domain-specific features are accurately captured and rendered, thereby greatly enhancing the system’s utility in scientific visualization tasks.

\textbf{Domain-Specific Fine-Tuning for Enhanced Feature Queries: Rajiv}
To ensure that Vizman Agent47 can accurately interpret and visualize domain-specific features, especially when new datasets are introduced, we incorporate a fine-tuning workflow for our locally deployed Llama-Vision model. This workflow is activated whenever a dataset containing novel or highly specialized features is added to the system. The fine-tuning process begins by collecting a representative sample of images from the new dataset, along with detailed annotations describing the key features of interest. These annotations serve as ground truth for the model, guiding it to recognize subtle, domain-specific patterns that are not well-represented in the general pre-trained model. Next, these images and annotations are formatted into a fine-tuning dataset, which is then used to update the Llama-Vision model. The training process involves adjusting the model's weights to improve its performance on these specific visual cues, thereby enhancing its ability to generate precise descriptions in response to natural language feature queries.

Once the model has been fine-tuned, it is seamlessly integrated back into the Vizman Agent47 workflow. The updated Llama-Vision model now provides improved analysis of screenshots, enabling more accurate extraction of isovalue recommendations and feature descriptions. This, in turn, enhances the overall reliability of the feature-based query system—ensuring that even for datasets with unique, domain-specific characteristics, the system can effectively interpret user requests and generate targeted visualizations. In summary, this domain-specific fine-tuning workflow is a critical component of Vizman Agent47. It ensures that as new datasets with specialized features are introduced, the system remains robust and continues to deliver high-quality, context-aware visualizations that meet the evolving needs of its users.


By combining detailed image analysis, a structured and continually updated knowledge base, and advanced LLM reasoning with a locally fine-tuned Llama-Vision model, Vizman Agent47 delivers a robust, context-rich approach to feature-based queries. This multi-step, data-driven process is a cornerstone of our contribution, setting a new standard for adaptive and feature-centric visualization workflows in the domain of high-performance scientific computing.

\subsubsection{Asynchronous Self-Improvement}

Vizman Agent47 is designed to continuously refine its performance and expand its capabilities through asynchronous self-improvement mechanisms that operate independently of direct user interactions. This self-improvement occurs in two distinct ways:

First, a background tool periodically scans the \texttt{code\_generation\_log.db} for any newly generated visualization code that has not yet been validated. For each unvalidated entry, the system automatically invokes the code validation and fixing module. This module executes the generated code, captures runtime outputs and errors, and—if necessary—iteratively applies fixes until the code meets the specified requirements. Once a piece of code is validated (either with no errors or with errors that have been fixed), the corresponding status flag in the database is updated. On subsequent user sessions, these validated code modules are integrated into the system's cache of pre-existing tools, which results in faster reaction times and a more robust overall pipeline.

Second, the screenshot generation process is itself designed to self-improve. The system continuously generates additional screenshots by exploring a wider range of isovalues and view angles for each dataset. As more images are captured, the associated keyword set describing the dataset’s features is incrementally expanded. This iterative process leverages feedback from the vision analysis modules to update and refine the descriptive metadata stored in the SQLite database. The self-improvement loop for screenshots halts once successive iterations yield no new keywords or significant changes in the visual features, ensuring that the knowledge base remains both comprehensive and efficient.

Together, these asynchronous self-improvement strategies ensure that Vizman Agent47 not only adapts to new datasets and evolving user queries over time but also maintains a high level of responsiveness and accuracy by continuously integrating validated code and enriched visual metadata into its workflow.


\subsubsection{Retrieval Augmented Generation (RAG) for In-Context Refinement}

Vizman Agent47 incorporates a lightweight Retrieval Augmented Generation (RAG) mechanism to enhance in-context learning during code generation. By retrieving relevant past interactions, user queries, and validated code snippets, this module provides additional context to the LLM, helping to suggest sensible default visualization parameters when explicit user input is lacking. Although the current implementation of RAG is not heavily leveraged for extensive validation, its role in augmenting the LLM's understanding of domain-specific subtleties is critical. This in-context refinement ensures that even when users provide minimal guidance, the system can generate visualization code that aligns well with established patterns and the overall design principles of the framework.


Overall, the integration of these components in Vizman Agent47 creates a robust, adaptive, and continuously improving visualization framework that addresses both routine tasks and sophisticated, domain-specific challenges. The methodology presented herein sets a new standard for agentic workflows in scientific visualization.

